Prescribed-Time Contracting-Boundary Control of a Tendon-Driven Flexible Arm

This study develops a prescribed-time performance-shaping control method for curvature tracking of a single-segment flexible arm actuated by three antagonistic tendon pairs. A Cartesian curvature representation is introduced to avoid the undefined bending direction at the straight configuration and to establish an explicit six-tendon kinematic mapping. A cubic performance boundary contracts smoothly from an initially admissible error bound to a nonzero terminal accuracy bound within a prescribed time. Based on this boundary, a dual transformation combining static symmetric error scaling and time-varying behavior shaping maps the tracking error into a fixed unit box. The resulting controller guarantees boundary invariance, prescribed-time entry into the terminal accuracy region, and subsequent asymptotic convergence. Numerical evaluations with Python and OpenCR--MuJoCo, together with a supervised reduced-order experiment on a two-section, four-channel platform, provide complementary validation. Across six experimental trials, no violation of the prescribed boundary is observed, and the proposed controller reduces the mean terminal curvature RMSE by 32.5% relative to a matched baseline, with comparable terminal-band entry times. These results support the feasibility of the proposed approach in the reduced-order experimental setting.

==> figures/fig_01a_geometry_3d.tex <==
% Reproducible panel (a): projected three-dimensional single-segment geometry.
% This file is intentionally limited to the first panel of Figure 2.

% Projected backbone stations. Elliptical guide sections and the oblique y axis
% provide depth cues without introducing a photorealistic rendering style.
\coordinate (Czero) at (2.06,0.78);
\coordinate (Cone)  at (2.04,1.53);
\coordinate (Ctwo)  at (2.17,2.32);
\coordinate (Cthree) at (2.55,3.08);
\coordinate (Cfour) at (3.26,3.78);

\def\PanelStation#1#2#3{%
  \begin{scope}[shift={#2},rotate=#3,xscale=1.00,yscale=0.34]
    \foreach \ang/\num in {0/1,60/2,120/3,180/4,240/5,300/6}{%
      \coordinate (#1\num) at (\ang:0.52);
    }
  \end{scope}%
}
\PanelStation{A}{(2.06,0.78)}{-8}
\PanelStation{B}{(2.04,1.53)}{-1}
\PanelStation{C}{(2.17,2.32)}{9}
\PanelStation{D}{(2.55,3.08)}{19}
\PanelStation{E}{(3.26,3.78)}{31}

% Base frame and undeformed center-axis reference.
\draw[->,black!70] (Czero)--++(0.94,-0.01)
  node[annotation,anchor=west] {\(+x\)};
\draw[->,black!70] (Czero)--++(-0.66,0.35)
  node[annotation,anchor=east] {\(+y\)};
\draw[->,black!55,densely dashed] (Czero)--(2.06,4.25)
  node[annotation,anchor=south] {undeformed \(+z\)};

% Curvature-vector projection in the base cross-sectional plane.
\draw[->,very thick,black!78] (Czero)--++(0.49,0.24);
\node[annotation,anchor=south west] at (2.39,1.00)
  {\(\vect c=[c_x,c_y]\trans\)};

% Smooth constant-curvature centerline.
\draw[very thick,black!72]
  plot[smooth,tension=0.62] coordinates
  {(Czero) (Cone) (Ctwo) (Cthree) (Cfour)};

% Six tendon paths. Pair colors and dash patterns match panel (b).
\foreach \num in {1,4}{%
  \draw[thick,red!60!black]
    plot[smooth,tension=0.62] coordinates
    {(A\num) (B\num) (C\num) (D\num) (E\num)};
}
\foreach \num in {2,5}{%
  \draw[thick,blue!62!black,dashed]
    plot[smooth,tension=0.62] coordinates
    {(A\num) (B\num) (C\num) (D\num) (E\num)};
}
\foreach \num in {3,6}{%
  \draw[thick,green!42!black,dash dot]
    plot[smooth,tension=0.62] coordinates
    {(A\num) (B\num) (C\num) (D\num) (E\num)};
}

% Perspective guide sections: dashed rear halves and solid front halves.
\def\PanelRing#1#2{%
  \begin{scope}[shift={#1},rotate=#2,xscale=1.00,yscale=0.34]
    \draw[black!28,densely dashed]
      (0.52,0) arc[start angle=0,end angle=180,radius=0.52];
    \draw[black!55]
      (-0.52,0) arc[start angle=180,end angle=360,radius=0.52];
  \end{scope}%
}
\PanelRing{(2.06,0.78)}{-8}
\PanelRing{(2.04,1.53)}{-1}
\PanelRing{(2.17,2.32)}{9}
\PanelRing{(2.55,3.08)}{19}
\PanelRing{(3.26,3.78)}{31}

% Distal tendon locations and numbering.
\foreach \num in {1,4}{\fill[red!60!black] (E\num) circle (0.045);}
\foreach \num in {2,5}{\fill[blue!62!black] (E\num) circle (0.045);}
\foreach \num in {3,6}{\fill[green!42!black] (E\num) circle (0.045);}
\node[annotation,anchor=west] at ($(E1)+(0.09,0.02)$) {1};
\node[annotation,anchor=south west] at ($(E2)+(0.02,0.07)$) {2};
\node[annotation,anchor=south east] at ($(E3)+(-0.02,0.07)$) {3};
\node[annotation,anchor=east] at ($(E4)+(-0.09,-0.01)$) {4};
\node[annotation,anchor=north east] at ($(E5)+(-0.02,-0.07)$) {5};
\node[annotation,anchor=north west] at ($(E6)+(0.02,-0.07)$) {6};

% Compact pair key and segment-length annotation.
\node[annotation,anchor=west] at (0.10,3.34) {antagonistic pairs};
\draw[thick,red!60!black] (0.16,3.08)--(0.62,3.08);
\node[annotation,anchor=west] at (0.69,3.08) {\((1,4)\)};
\draw[thick,blue!62!black,dashed] (0.16,2.80)--(0.62,2.80);
\node[annotation,anchor=west] at (0.69,2.80) {\((2,5)\)};
\draw[thick,green!42!black,dash dot] (0.16,2.52)--(0.62,2.52);
\node[annotation,anchor=west] at (0.69,2.52) {\((3,6)\)};

\node[annotation,anchor=west] (Llabel) at (4.24,2.75)
  {centerline \(L\)};
\draw[->,black!52] (Llabel.west)--(2.70,3.18);

\node[paneltitle,anchor=base] at (2.90,-0.24)
  {\textbf{(a)} 3D single-segment tendon-driven geometry};

